Manipulator as a Tail: Promoting Dynamic Stability for Legged Locomotion

For locomotion, is an arm on a legged robot a liability or an asset for locomotion? Biological systems evolved additional limbs beyond legs that facilitates postural control. This work shows how a manipulator can be an asset for legged locomotion at high speeds or under external perturbations, where the arm serves beyond manipulation. Since the system has 15 degrees of freedom (twelve for the legged robot and three for the arm), off-the-shelf reinforcement learning (RL) algorithms struggle to learn effective locomotion policies. Inspired by Bernstein's neurophysiological theory of animal motor learning, we develop an incremental training procedure that initially freezes some degrees of freedom and gradually releases them, using behaviour cloning (BC) from an early learning procedure to guide optimization in later learning. Simulation experiments show that our policy increases the success rate by up to 61 percentage points over the baselines. Simulation and real robot experiments suggest that our policy learns to use the arm as a tail to initiate robot turning at high speeds and to stabilize the quadruped under external perturbations. Quantitatively, in simulation experiments, we cut the failure rate up to 43.6% during high-speed turning and up to 31.8% for quadruped under external forces compared to using a locked arm.

==> RSS_citation_info.tex <==
\section{RSS citations}

Please make sure to include \verb!natbib.sty! and to use the
\verb!plainnat.bst! bibliography style. \verb!natbib! provides additional
citation commands, most usefully \verb!\citet!. For example, rather than the
awkward construction 

{\small
\begin{verbatim}
\cite{kalman1960new} demonstrated...
\end{verbatim}
}

\noindent
rendered as ``\cite{kalman1960new} demonstrated...,''
or the
inconvenient 

{\small
\begin{verbatim}
Kalman \cite{kalman1960new} 
demonstrated...
\end{verbatim}
}

\noindent
rendered as 
``Kalman \cite{kalman1960new} demonstrated...'', 
one can
write 

{\small
\begin{verbatim}
\citet{kalman1960new} demonstrated... 
\end{verbatim}
}
\noindent
which renders as ``\citet{kalman1960new} demonstrated...'' and is 
both easy to write and much easier to read.
  
\subsection{RSS Hyperlinks}

This year, we would like to use the ability of PDF viewers to interpret
hyperlinks, specifically to allow each reference in the bibliography to be a
link to an online version of the reference. 
As an example, if you were to cite ``Passive Dynamic Walking''
\cite{McGeer01041990}, the entry in the bibtex would read:

{\small
\begin{verbatim}
@article{McGeer01041990,
  author = {McGeer, Tad}, 
  title = {\href{http://ijr.sagepub.com/content/9/2/62.abstract}{Passive Dynamic Walking}}, 
  volume = {9}, 
  number = {2}, 
  pages = {62-82}, 
  year = {1990}, 
  doi = {10.1177/027836499000900206}, 
  URL = {http://ijr.sagepub.com/content/9/2/62.abstract}, 
  eprint = {http://ijr.sagepub.com/content/9/2/62.full.pdf+html}, 
  journal = {The International Journal of Robotics Research}
}
\end{verbatim}
}
\noindent
and the entry in the compiled PDF would look like:

\def\tmplabel#1{[#1]}

\begin{enumerate}
\item[\tmplabel{1}] Tad McGeer. \href{http://ijr.sagepub.com/content/9/2/62.abstract}{Passive Dynamic
Walking}. {\em The International Journal of Robotics Research}, 9(2):62--82,
1990.
\end{enumerate}
%
where the title of the article is a link that takes you to the article on IJRR's website. 


Linking cited articles will not always be possible, especially for
older articles. There are also often several versions of papers
online: authors are free to decide what to use as the link destination
yet we strongly encourage to link to archival or publisher sites
(such as IEEE Xplore or Sage Journals).  We encourage all authors to use this feature to
the extent possible.

==> figures/real_gait.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{figures/real_gait.png}
    \caption{We analyze the behavior of our policy when disturbed by a moving incline. We plot the rotation on the roll axis, as well as the third and fourth components of the extrinsic vector $z_t$ predicted by the estimator module. When the plank moves, we see a change in the extrinsic vector, indicating that the disturbance has been detected. The change in extrinsic triggers the reaction of the arm, which moves in the opposite direction to the plank to generate angular momentum. Such momentum helps to keep the roll of the robot constant during the disturbance.
    }
    \label{fig:gait}
\end{figure*}

==> sections/seed0.tex <==
\begin{table*} [h!]
\begin{center}
\vspace{-10pt}
 \begin{tabular}{ c||cc cc cc}
\multirow{2}{*}{Arm} & \multicolumn{2}{c}{\textbf{Success \%} ($\uparrow$)} & \multicolumn{2}{c}{\textbf{TTF \%} ($\uparrow$) } & \multicolumn{2}{c}{\textbf{$V_{lin}$ Tracking Error} ($\downarrow$)}\\
\cline{2-7}
 & 200-300& 300-400 & 200-300& 300-400 & 200-300& 300-400\\
 \hline
No Arm  & 95.80 & 66.30 & \textbf{0.980}$\pm$0.11& 0.795$\pm$0.31   & 0.234$\pm$0.03& 0.755$\pm$0.02 \\
Locked  & 89.50& 45.75  & 0.945$\pm$0.18& 0.628$\pm$0.36   & 0.068$\pm$0.00& 0.225$\pm$0.01 \\
Actuated&\textbf{96.00}& \textbf{80.00} & 0.977$\pm$0.12&\textbf{0.878}$\pm$0.26   & \textbf{0.026}$\pm$0.00& \textbf{0.119}$\pm$0.01\\
\end{tabular}
\end{center}
\caption{Simulation comparison for stable locomotion with and without an actuated arm.}
\label{tab:results_set1_appendix}
\vspace{-10pt}
\end{table*}

\begin{table*} [h!]
\begin{center}
 \begin{tabular}{c| c|cccccc}
$V_{lin}$ Command & Arm & \textbf{Success \%} ($\uparrow$)  &  \textbf{$V_{ang}$  Error}($\downarrow$) & \textbf{$V_{lin}$  Error} ($\downarrow$) \\
 \hline
\multirow{3}{*}{1 $m/s$}&No Arm & \textbf{89.80}  & 0.332$\pm$0.022  & 0.015$\pm$0.001\\
&Locked & 83.15  & 0.241$\pm$0.013  & 0.015$\pm$0.001\\
&Actuated & 89.45 & \textbf{0.183}$\pm$0.012  & \textbf{0.009}$\pm$0.001\\
\hline
\multirow{3}{*}{1.25 $m/s$}&No Arm & \textbf{88.65}& 0.301$\pm$0.019  & 0.022$\pm$0.001 \\
&Locked  & 78.65 & 0.222$\pm$0.010 & 0.024$\pm$0.001  \\
&Actuated   & 87.85 & \textbf{0.179}$\pm$0.011 & \textbf{0.015}$\pm$0.001\\
\hline
\multirow{3}{*}{1.5 $m/s$}&No Arm & \textbf{85.75}  & 0.294$\pm$0.016  & 0.032$\pm$0.001\\
&Locked  & 69.60 & 0.223$\pm$0.008 & 0.036$\pm$0.001 \\
&Actuated   & 83.75 & \textbf{0.175}$\pm$0.009 & \textbf{0.024}$\pm$0.001\\
\end{tabular}
\end{center}
\caption{Simulation evaluation for turning at high speed. 
% Velocities are sampled at $1$, $1.25$ and $1.5$ $m/s$. Across all velocities, our method with the arm actuated always outperforms our method with the arm locked, across the success rate, angular velocity tracking, and linear velocity tracking. 
}
\label{tab:results_turn_appendix}
\vspace{-10pt}
\end{table*}
